Vehicle Teleoperation: Successive Reference-Pose Tracking

Vehicle teleoperation is an interesting feature in many fields. A typical problem of teleoperation is communication time delay which, together with actuator saturation and environmental disturbance, can cause a vehicle deviation from the target trajectory imposed by the human operator who imposes to the vehicle a steering wheel angle reference and a speed/acceleration reference. With predictive techniques, time-delay can be accounted at sufficient extent. But, in presence of disturbances, due to the absence of instantaneous haptic and visual feedback, human-operator steering command transmitted to the the vehicle is unaccounted with disturbances observed by the vehicle. To improve reference tracking without losing promptness in driving control, reference trajectory in the form of successive reference poses can be transmitted instead of steering commands to the vehicle. We introduce this new concept, namely, the 'successive reference-pose tracking (SRPT)' to improve path tracking in vehicle teleoperation. This paper discusses feasibility and advantages of this new method, compare to the smith predictor control approach. Simulations are performed in SIMULINK environment, where a 14-dof vehicle model is being controlled with Smith and SRPT controllers in presence of variable network delay. Scenarios for performance comparison are low adhesion ground, strong lateral wind and steer-rate demanding maneuvers. Simulation result shows significant improvement in reference tracking with SRPT approach.

==> sections/02-method2_varDelay.tex <==
\subsection{Simulating variable network delay in Simulink}
How to simulate variable network delays in Simulink? Zhang and Yeddanapudi \cite{Zhang2012ModelingAS} suggests not to use block \textit{Variable transport delay} in context of network control system because it relates to physical processes where a medium is transported with a specified speed. Steinberger et al. \cite{Martin2020} suggests that the desired delay should not directly be used as an input signal to the block \textit{Variable Integer Delay}. Instead they proposed an algorithm, which can be used to link the packets to the desired packet delays, which extends the Simulink built-in block to achieve accurate simulation results. An instinctive approach to simulate Variable time-delays is to exploit the Simulink built-in blocks \textit{Variable time delay}. It has two in-ports; input signals $u(t)$ and time delay input $t_d(t)$, as shown in bottom right area of fig (\ref{fig:07_variableDelaySim}a). Using approach given in previous subsection, sequence of downlink-delays ($\tau_{2,1:n}$) can be obtained. This sequence guarantees FIFO fashion reception of data packets at the receiver end. Considering FIFO ordered data packets, table \ref{tab:timeDelayInputSimulink} proposes the random saw tooth profile of $t_d(t)$ signal given in fig (\ref{fig:07_variableDelaySim}b). In order to validate the effectiveness of this profile, a sample case of data packets associated to variable network delays is used as a ground truth to be tested upon. In this case, data packets $1:8$ are transmitted by the sender and received by the receiver after associated variable delays to them, fig (\ref{fig:dataPktsGroundTru}). 

\begin{figure}[h]
\centering
    \includegraphics[width=0.8\columnwidth,cfbox=black .1pt .1pt]{figures/06_variableDelaySim.eps}
    \caption{A network delay case to be simulated (Ground truth)}
    \label{fig:dataPktsGroundTru}%
\end{figure}

\begin{table}[h]
\centering
\caption{Data packets and their delays (Ground truth)}
\begin{tabular}{|c|c|c|c|}
\hline
\multicolumn{1}{|l|}{\textbf{Data pkt (n)}} & \multicolumn{1}{l|}{{\color[HTML]{0000FF} \textbf{DT_n}}} & \multicolumn{1}{l|}{\textbf{Delay ($\tau_{2,n}$)}} & \multicolumn{1}{l|}{{\color[HTML]{D40000} \textbf{AT_n}}} \\ \hline
1                                           & 0                                                         & 2.5                                                & 2.5                                                       \\ \hline
2                                           & 1                                                         & 2                                                  & 3                                                         \\ \hline
3                                           & 2                                                         & 2                                                  & 4                                                         \\ \hline
4                                           & 3                                                         & 1.5                                                & 4.5                                                       \\ \hline
5                                           & 4                                                         & 1                                                  & 5                                                         \\ \hline
6                                           & 5                                                         & 1.5                                                & 6.5                                                       \\ \hline
7                                           & 6                                                         & 1                                                  & 7                                                         \\ \hline
8                                           & 7                                                         & 1                                                  & 8                                                         \\ \hline
\end{tabular}
\label{tab:dataPktsGroundTru}
\end{table}

Table \ref{tab:dataPktsGroundTru} reports the departure time (DT) and delay associated to each data packet of the sample case. As data packet DTs and corresponding delay sequence are prior known, associated arrival times (ATs) are computed and listed in column 4 of table \ref{tab:dataPktsGroundTru}. Which is then to be used to prepare the saw tooth profile of $t_d(t)$ signal in table \ref{tab:timeDelayInputSimulink}. Column 1 of table \ref{tab:timeDelayInputSimulink} lists the domain of the $t_d(t)$ profile and column 2 lists the corresponding range.

\begin{table}[h]
\centering
\caption{Time-delay input for Simulink \textit{Variable time delay}}
\begin{tabular}{|l|l|}
\hline
\textbf{Simulation time, $t$} & \textbf{Time-delay input, $t_d(t)$}             \\ \hline
[0\:\:\:\:\:\:\:\:\:\:\:, AT_1)                   & \:\:\tau_{2, 1}                           \\ \hline
[AT_1\:\:\:\:\:, AT_2)                & [\tau_{2, 1}\:\:\:\:\:, \Delta T+\tau_{2, 2})   \\ \hline
[AT_2 \:\:\:\:\:, AT_3)                & [\tau_{2, 2}\:\:\:\:\:, \Delta T+\tau_{2, 3})   \\ \hline
\multicolumn{1}{|c|}{|}     & \multicolumn{1}{c|}{|}                \\ \hline
[AT_{n-1}, AT_{n})          & [\tau_{2, n-1}, \Delta T+\tau_{2, n}) \\ \hline
\:\:AT_{n}                      & \:\:\tau_{2, n}                           \\ \hline
\end{tabular}
\label{tab:timeDelayInputSimulink}
\end{table}

To simulate varying network delays given of fig (\ref{fig:dataPktsGroundTru}), data packets as per their DTs and $t_d(t)$ profile is fed to the block \textit{Variable time delay}. Fig (\ref{fig:07_variableDelaySim}a) compares output of the block and the ground truth. Exact match of simulation and ground truth validates the proposed $t_d(t)$ profile. Further to simulate discrete receive of vehicle states, control-station block (H in fig \ref{fig:smith_1}-\ref{fig:mpcScheme}) is treated as enabled subsystem, which is enabled only when the output of block \textit{variable time delay} is new. 

\begin{figure}[h]
\centering
    \includegraphics[width=\columnwidth]{figures/07_variableDelaySim_inkscape.eps}
    \caption{Input and output of \textit{Variable time delay} block}
    \label{fig:07_variableDelaySim}%
\end{figure}


==> sections/09-bios.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{JaiPrakash.png}}]%
{Jai Prakash}
was born in Delhi, India in 1990. He received the B.Tech. degree in Production Engineering from the National institute of technology, Trichy, India in 2012 and M.S. degree in Mechanical Engineering from the Politecnico di Milano, Italy in 2018. From 2018 to 2019, he was a research assistant in Mechanical Engineering Department of Politecnico di Milano. Since 2019, he is a doctoral candidate in Mechanical Engineering Department of Politecnico di Milano. His research interests include computer-vision, robotics, and vehicle dynamics.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{mic.jpg}}]%
{Michele Vignati}
received his M.S. degree (2013) and PhD (2017) in Mechanical Engineering from Politecnico di Milano with thesis on control strategies for distributed powertrain of hybrid and electric vehicles. From 2019 he is Assistant Professor (RTDA) in the research field of applied mechanics. In particular, he focuses on mechanical systems dynamics and control applied in the automotive field of which he has more than 20 publications in international journals and conferences. In 2018 he won the best paper award for a paper presented at the AVEC’18 international conference. He worked on tire dynamics and modelling in cooperation with Pirelli. He works in autonomous driving field and in vehicle modelling, testing, state estimation, and active control systems.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{edo.png}}]%
{Edoardo Sabbioni}
received his PhD in Mechanical Systems Engineering in 2007 and currently works as Associate Professor at the Department of Mechanical Engineering of Politecnico di Milano. His main research activities are in the field of stability, dynamics and control of mechanical systems, with applications to road and rail vehicles. He is also involved in research activities within the fields of aerodynamics and mechatronics. More in particular, he carried out numerical-experimental researches concerned with active safety of vehicles, design of control systems to improve vehicle handling and ride comfort, design of HiL (Hardware-in-the-Loop) test benches, electric and hybrid electric vehicles, autonomous and connected vehicle, “smart” tires technology, cross wind on road/rail vehicles. He is an author of more than 140 scientific publications, most of which published on peer-reviewed journals or presented at international conferences and he is a member of the Editorial Board of Shock and Vibration.

During his research activity, he cooperated and still cooperates with the main Italian automotive/railway industries and he was involved in several Italian and EC funded projects.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{cheli.jpg}}]%
{Federico Cheli}
received the M.S. degree in mechanical engineering from the Politecnico di Milano, Milano, Italy, in 1981. He is currently a Full Professor at the Department of Mechanical Engineering, Politecnico di Milano and author of more than 380 publications on international journals and conferences. His scientific activity concerns research on vehicle performance, handling and comfort problems, active control, ADAS, and electric and autonomous vehicles. He is a member of the editorial board of the International Journal of Vehicle Performance and International Journal of Vehicle Systems Modeling and Testing.
\end{IEEEbiography}
